Social Robot Navigation through Constrained Optimization: a Comparative Study of Uncertainty-based Objectives and Constraints

This work is dedicated to the study of how uncertainty estimation of the human motion prediction can be embedded into constrained optimization techniques, such as Model Predictive Control (MPC) for the social robot navigation. We propose several cost objectives and constraint functions obtained from the uncertainty of predicting pedestrian positions and related to the probability of the collision that can be applied to the MPC, and all the different variants are compared in challenging scenes with multiple agents. The main question this paper tries to answer is: what are the most important uncertainty-based criteria for social MPC? For that, we evaluate the proposed approaches with several social navigation metrics in an extensive set of scenarios of different complexity in reproducible synthetic environments. The main outcome of our study is a foundation for a practical guide on when and how to use uncertainty-aware approaches for social robot navigation in practice and what are the most effective criteria.

==> eval_draft.tex <==
\section{Evaluations}\label{sec_eval}

\subsection{Experimental setup}

Here we describe how we worked with experiments: describe the PyMiniSim environment, which models we have, describe robots kinematics, describe sensors, and etc. We describe here our approach for generating scenes. 

Discrete Unicycle Model:
\[
 \begin{matrix}
  x_{k+1} = x_{k} + v \cdot cos(\theta_{k}) \cdot \delta t \\
  y_{k+1} = y_{k} + v \cdot sin(\theta_{k}) \cdot \delta t \\
  \theta_{k+1} = \theta_{k} + w \cdot \delta t
 \end{matrix}
\]

\subsection{Methods}

Here we again briefly describe our controllers and give them names, also describe their parameters. Probably describe some other technical details if needed.
List of the controllers:
\begin{itemize}
    \item \textbf{ED-MPC} -  Euclidean Distance (additional component to the cost function) - Model Predictive Control. Classical cost function described in the chapter 2 with additional component to the cost function of Euclidean Distance to each of the pedestrian at the each propagation step. This controller does not count onto the propagated covariances of the CovarianceNET.
    \item \textbf{ED-MPC-EDC} - Euclidean Distance (additional component to the cost function) - Model Predictive Control - Euclidean Distance Constraint.
    \item \textbf{ED-MPC-MDC} - Euclidean Distance (additional component to the cost function) - Model Predictive Control - Mahalanobis Distance Constraint. This controller utilizes CovarianceNET for calculating Mahalanobis Distance to each of the pedestrian.
    \item \textbf{MD-MPC-EDC }- Mahalanobis Distance (additional component to the cost function) - Model Predictive Control - Euclidean Distance Constraint.
    \item \textbf{MD-MPC-MDC }- Mahalanobis Distance (additional component to the cost function) - Model Predictive Control - Mahalanobis Distance Constraint.
\end{itemize}

Here we describe common settings that all the controllers share with each other:
\begin{itemize}
    \item \(N = 25\), horizon steps, include the terminal step, [№];
    \item \(R = \left(\begin{smallmatrix}
     1&0 \\ 0&1
     \end{smallmatrix} \right)\), control input weighted matrix;
    \item \(v_{min} = 0\), minimum velocity bound, \([\frac{m}{s}]\);
    \item \(v_{max} = 2\), maximum velocity bound, \([\frac{m}{s}]\);
    \item \(\omega_{min} = -2\), minimum velocity bound, \([\frac{rad^2}{s}]\);
    \item \(\omega_{max} = 2\), maximum velocity bound,  \([\frac{rad^2}{s}]\);
    \item \(t_{ghost} = 20\), amount of controller steps to track ghost pedestrians, [№];
\end{itemize}
All controllers use the same standard \textit{do-mpc} solver \textit{MUltifrontal Massively Parallel sparse direct Solver (MUMPS)}.
However,  it is also possible to install additional solver package Coin-HSL. 
According to the research of \cite{tasseff2019exploring}, best HSL solvers (MA27 and MA57) have comparative performance. 
Thus, we have chosen free licensed standard MUMPS solver.

Here we describe common environment and robot settings:
\begin{itemize}
    \item \(d_{vis} = 5\), robot vision distance,\( [m]\);
    \item \(r_{rob} = 0.35\) , robot circumference radius,\( [m]\);
    \item \(r_{ped} = 0.3\) , pedestrian circumference radius, \([m]\);
    \item \(d_{safe}= 0.75\), minimum safe distance between the centers of mass of the agents, \([m]\);
    \item \(f_{vis} = \pi\),  field of view, [rad];
    \item \(d_{tol} = 0.3\), tolerance distance for subgoal reachability,[m];
    \item \(t_{simlimit} = 2000\), maximum amount of simulation steps, to run an experiment, \([\#]\);
    \item \(\Delta t_{sim} = 0.01\), time delta for a simulation step, \([\#]\);
    \item \(\Delta t_{control} = 0.1\), time delta for a controller step, \([\#]\);
\end{itemize}
Robot is \textit{not visible} for pedestrians. In all the experiments we used Optimal Reciprocal Collision Avoidance (ORCA) \cite{orca}  model for the pedestrians.

\begin{table}[]
\centering
\caption{Settings for different MPC variations }
\label{tab:mpc-settings}
\begin{tabular}{|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{}                                    & $\delta$ & Q    & W    \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{1F77B4} ED-MPC}     & -        & 1000 & 500  \\ \hline
{\color[HTML]{FF7F0E} ED-MPC-EDC}                         & 0.3      & 1000 & 500  \\ \hline
\cellcolor[HTML]{FFFFFF}{\color[HTML]{2CA02C} ED-MPC-MDC} & 2        & 1000 & 500  \\ \hline
{\color[HTML]{D62728} MD-MPC-EDC}                         & 0.3      & 100  & 1000 \\ \hline
{\color[HTML]{9467BD} MD-MPC-MDC}                         & 2        & 100  & 1000 \\ \hline
\end{tabular}
\end{table}

Also we describe here the architecture of our evaluation network. Also we can describe the CovarianceNet briefly here, how it was trained on SDD.

We also describe here how evaluation network was trained.

\subsection{Simulation Environment}
To run the experiments, we have developed a lightweight simulator called PyMiniSim (picture). (Dont know what to put more here).

\subsection{Experiment Preparation}
Before we continue with the explanation of scenario generation, it is necessary to emphasize several definitions:
\begin{itemize}
    \item \textbf{Common Sampling Area} - An available geometric space for the distribution of initial states and target positions for pedestrians and robots. It is a square of 8 m length, distributed from -4 to 4 for each of the coordinates.
    \item \textbf{Robot Local Goal Condition} - The local goal of the robot should be randomly sampled in the following range:
\[d_{min} \leq ||p_i - subgoal||_{2} \leq N \cdot v_{max} \cdot \delta t + \epsilon\]
where: \(d_{min}\) - minimum sampling distance, \(p_i\) - sampled initial robot position, \(subgoal\) - sampled robot subgoal position, \(N\) - controller horizon steps, \(v_{max}\) - maximum forward velocity, \(\delta t\) - controller time step, \(\epsilon\) - range constant to adjust the maximum sampling distance.
\end{itemize}
To evaluate the proposed methods, we have prepared several scenarios:
\begin{itemize}
    \item \textbf{Circular Crossing Scenario} - The initial states of the pedestrians are randomly distributed around the ring of the inner radius \(r_{inner}\) and the outer radius of \(r_{outer}\).  They are distributed so that they do not collide with each other when they are spawned. The pedestrians end positions are opposite to the initial states, crossing the center of the ring. Robot's start position belongs to the circle of radius \(r_{inner}\).  The robot's target position is randomly distributed around the common sampling area, according to the robot's local goal condition.
    \item \textbf{Random Crossing Scenario} - Pedestrians and robot initial states and finish positions are randomly distributed around the playing area. They are distributed so as not to collide with each other when they are spawned. The robot's target position is randomly distributed around the common sampling area, according to the robot's local goal condition.
    \item \textbf{Parallel Crossing Scenario} - The initial states of the pedestrians are distributed on opposite sides of the common sampling area, and their target positions are on the opposite side. Pedestrians move towards each other. The robot's initial state is sampled in the middle of the way of the pedestrians, and its target position is sampled according to the rule of the robot local goal condition.
\end{itemize}
For better visual understanding, refer to the figure \ref{scenario_generation}. It is necessary to mention that after the pedestrians reach their target positions, they go back to the starting position and oscillate back and forth until the experiment is over.

% Scenario Generator
\begin{figure*}
  \includegraphics[width=\textwidth]{fig/scenario_generation.png}
  \caption{Scenario Generation}
  \label{scenario_generation}
\end{figure*}

\subsection{Results and analysis}

To collect the statistical data we have run 1800 experiments for each of the controller. After the data has been collected, we shaped statistical results. We have chosen 3 metrics to evaluate the performance of the proposed methods:
\begin{itemize}
    \item \textbf{Simulation Steps to Subgoal,  \([\#]\)} - Time proportional metric, it shows how conservative the controller is;
    \item \textbf{Number of Collisions,  \([\#]\)} - The metric shows the amount of collisions between the robot and pedestrians during the experiment, the less the amount of collisions - the more safe the controller is;
    \item \textbf{Number of Timeouts,  \([\#]\)} - The metric shows if the amount of simulations steps was exceeded \(t_{simlimit}\). Experiments with timeouts did not take into account for \textbf{Simulation Steps to Subgoal} metric.
\end{itemize}

\textbf{Do we need a separate analysis on global goal for MPC methods then?}

Here we put the results. Probably, show how controllers perform for global goal, then show how network predicts the evaluation of the goal. Then we also try to do sampling with evaluation.

% Circular Crossing
\begin{figure*}
  \includegraphics[width=\textwidth]{fig/circular_crossing_graph.png}
  \caption{Circular Crossing}
  \label{circular_crossing}
\end{figure*}

% Random Crossing
\begin{figure*}
  \includegraphics[width=\textwidth]{fig/random_crossing_graph.png}
  \caption{Random Crossing}
  \label{random_crossing}
\end{figure*}

% Parallel Crossing
\begin{figure*}
  \includegraphics[width=\textwidth]{fig/parallel_crossing_graph.png}
  \caption{Parallel Crossing}
  \label{parallel_crossing}
\end{figure*}

And finally we discuss our next direction with subgoal recommendation.

==> method_draft.tex <==
\section{Proposed methods}

\textbf{FULL LIST OF NOTATION USED IN THE PAPER:}
\begin{itemize}
    \item[] \(x^{robot}\) - position of the robot along \(x \) axis, \([m]\);
    \item[] \(y^{robot}\) - position of the robot along \(y \) axis, \([m]\);
    \item[] \(\theta^{robot}\) - angular position of the robot, \([rad]\);
    \item[] \(v^{robot}\) - linear velocity of the robot, \([\frac{m}{s}]\);
    \item[] \(\omega^{robot}\) - angular velocity of the robot, \([\frac{rad}{s}]\);
    \item[] \(x^{ped}_{k_{c} | i}\) -  \textit{i}-th pedestrian position along \(x \) axis, \([m]\);
    \item[] \(y^{ped}_{k_{c} | i}\) -  \textit{i}-th pedestrian position along \(y \) axis, \([m]\);
    \item[] \(v_x^{ped}\) - pedestrian linear velocity along \(x\) axis, \([\frac{m}{s}]\);
    \item[] \(v_y^{ped}\) - pedestrian linear velocity along \(y\) axis, \([\frac{m}{s}]\);
    \item[] \(k\) - time step, \([\#]\);
    \item[] \(k_{s}\)- simulation step, \([\#]\);
    \item[] \(k_{c}\)- controller step, \( \quad k_{c}=\{0,1, \ldots, N-1\}\), \([\#]\);
    \item[] \(\Delta t\) - time step interval, \([s]\);
    \item[] \(\Delta t_{s}\) - simulation time step interval, \([s]\);
    \item[] \(\Delta t_{c}\) - controller time step interval, \([s]\);
    \item[] \(N\) - controller number of horizon steps, \([\#]\);
    \item[] \(N^{ped}\) - number of pedestrians, \([\#]\);
    \item[] \(Q_{\mathbf{u}}\) - control input weighted matrix;
    \item[] \(Q_{\mathbf{r}}\) - normalized position penalty weight scalar coefficient;
    \item[] \(Q_{\mathbf{ED}}\) - Euclidean distance cost weight;
    \item[] \(Q_{\mathbf{MD}}\) - Mahalanobis distance cost weight;
    \item[] \(c^{\mathbf{ED}}_{k_{c} | i}\) - constraint value for Euclidean distance constraint for \(i\)-th pedestrian at the \(k_{c}\) receding horizon step;
    \item[] \(c^{\mathbf{MD}}_{k_{c} | i}\) - constraint value for Mahalanobis distance constraint;
    \item[] \(\delta^{\mathbf{ED}}\) - adaptive constraint value for Euclidean distance constraint;
    \item[] \(\delta^{\mathbf{MD}}\) - adaptive constraint value for Mahalanobis distance constraint;
    \item[] \(\mathbf{r}^{target}\) - robot target position point;
    \item[] \(\mathbf{r}_{0}\) - initial robot position at the each iteration of the MPC;
    \item[] \(\mathbf{r}_{k_{c}}\) - \(k_{c}\)-th robot position inside MPC horizon propagation;
    \item[] \(\mathbf{r} = [x^{robot}, y^{robot}]\) - robot position vector;
    \item[] \(\mathbf{x} = [x^{robot}, y^{robot}, \theta^{robot}]\) - robot state vector;
    \item[] \(\mathbf{u} = [v^{robot}, \omega^{robot}]\) - robot input vector;
    \item[] \(\mathbf{p}^i_{k_{c}} = [x_{k_{c} | i}^{ped}, y_{k_{c} | i}^{ped}]\) -  \textit{i}-th pedestrian position vector at the controller step \(k_{c}\),  \( \quad i=\{1, \ldots, N^{ped}\}\); 
    \item[] \(\mathcal{U} \)- action space;
    \item[]\( \mathcal{S} \)- state space;
    \item[] \(r^{ped}\) - pedestrian circumference radius;
    \item[] \(r^{robot}\) - robot circumference radius;
    \item[] \(d^{safe}\) - safe distance between robot and pedestrian circumferences;
\end{itemize}



\subsection{System description}

Before explaining the proposed MPC recipes, let us introduce system dynamics. Since it is a crucial constraint for the behavior of the system to follow a deterministic Markov decision process.  As a dynamic model for the robot, we have chosen a unicycle model and we have represented it as a discrete system. The unicycle model is the simplest representation of the differential drive kinematics, which is an advantage of the model. Its disadvantage is the lack of dynamic parameters such as inertia or friction coefficients. However, optimal control methods such as MPC can handle such variations when implemented on the real robotic platform.

\textbf{Robot dynamics: Discrete Unicycle Model}
\begin{equation} 
     \begin{matrix}
          x^{robot}_{k+1} = x^{robot}_{k} + v^{robot} \cdot cos(\theta^{robot}_{k}) \cdot \Delta t \\
          y^{robot}_{k+1} = y^{robot}_{k} + v^{robot} \cdot sin(\theta^{robot}_{k}) \cdot \Delta t \\
          \theta^{robot}_{k+1} = \theta^{robot}_{k} + w^{robot} \cdot \Delta t
     \end{matrix}
\end{equation}

Note that with a difference in time step intervals between these entities, this model is used as a simulation model for Model Predictive Control.
For the pedestrian model, we have used a Headed Social Force Model \cite{HSFM}, which is a very well-known model for the simulation of pedestrian behavior.

% \begin{equation} \label{eq:system_dynamics}
%  \begin{matrix}
%   x_{k+1} = x_{k} + v \cdot cos(\theta_{k}) \cdot \Delta t \\
%   y_{k+1} = y_{k} + v \cdot sin(\theta_{k}) \cdot \Delta t \\
%   \theta_{k+1} = \theta_{k} + w \cdot \Delta t
%  \end{matrix}
% \end{equation}
% where:
% \begin{itemize}
%     \item[] \(x\) - position of the robot along \(x \) axis, \([m]\);
%     \item[] \(y\) - position of the robot along \(y \) axis, \([m]\);
%     \item[] \(\theta\) - angular position of the robot, \([rad]\);
%     \item[] \(v\) - linear velocity of the robot, \([\frac{m}{s}]\);
%     \item[] \(\omega\) - angular velocity of the robot, \([\frac{rad}{s}]\);
%     \item[] \(k\) - simulation step, \([\#]\);
%     \item[] \(\Delta t\) - time step interval, \([s]\);
% \end{itemize}

% Hence the full state vector of the system is: \(\mathbf{x} = [x, y, \theta]\), control input vector is: \(\mathbf{u} = [v, \omega]\). In addition it is required to introduce position coordinate vector: \(\mathbf{p} = [x, y]\), since in the used cost function we do not use a penalty on angular position of the robot.

\subsection{Uncertainty-aware social costs and constraints}

In this section we will describe all the methods that we have investigated. The core of each of the methods is a Model Predictive Control method. The cost function consisted of two parts: \textit{stage cost} and\textit{ terminal cost}. The stage cost is cost that accumulated at the each stage of the prediction horizon until the very last step called terminal step. The stage cost also consist of two parts: \textit{control input cost} and \textit{normalized target point distance cost}. 

\textbf{The control input cost function}:
\begin{equation} \label{}
J_{k_{c}}^{\mathbf{u}}\left(\mathbf{u}_{k_{c}}\right) = \mathbf{u}^T_{k_{c}} Q_{\mathbf{u}} \mathbf{u}_{k_{c}}
\end{equation}
where:
% \begin{itemize}
%     \item[] \(Q_{\mathbf{u}}\) - control input weighted matrix;
%     \item[] \(N\) - amount of horizon steps;
% \end{itemize}

In fact, this part of the stage cost function penalizes utilization of the 

\textbf{The normalized target point distance cost}:
\begin{equation} \label{eq:}
J_{k_{c}}^{\mathbf{r}}\left(\mathbf{r}_{k_{c}}\right)= Q_{\mathbf{r}}
\left(    \frac{ \left\| \mathbf{r}_{k_{c}} - \mathbf{r}_{target} \right\|_2 } 
         { \left\| \mathbf{r}_0 - \mathbf{r}_{target} \right\|_2} \right)^2
\end{equation}
% where:
% \begin{itemize}
%     \item[] \(Q_{\mathbf{p}}\) - normalized position penalty weight scalar coefficient;
%     \item[]  \(\mathbf{p}^{target}\) - target position point;
% \end{itemize}

In other words, this term reflects \textit{how far we got at \(k\) simulation step in comparison to the initial position at the beginning of the MPC computation}. This cost function has some drawbacks, such as the homotopy equivalence effect. In such situations, the controller cannot decide which way to run until an external factor, such as a pedestrian, affects the position of the robot \ref{fig:homotopy}. This effect will be fixed by the implementation of the subgoal recommendation system.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/Homotopy.png}
    \caption{a) The robot is experiencing the homotopy equivalence effect.  The robot will not move until pedestrian circled in red will affect his position. b) The robot's position was affected by the propagated covariance of the marked pedestrian and now it has started to move towards the goal.}
    \label{fig:homotopy}
\end{figure}


Hence,  \textbf{the stage cost function} is a sum of this two functions:

\begin{equation}
J_{k_{c}} (\mathbf{u}_{k_{c}}, \mathbf{r}_{k_{c}}) = J_{k_{c}}^{\mathbf{u}}\left(\mathbf{u}_{k_{c}}\right) + J_{k_{c}}^{\mathbf{r}}\left(\mathbf{r}_{k_{c}}\right)
\end{equation}

\textbf{The terminal cost} is the cost at the very last step of the prediction horizon and we include only the normalized target point distance cost at the very last stage:
\begin{equation} 
J_{N}\left(\mathbf{r}_{N}\right)= Q_{\mathbf{r}}
\left(    \frac{ \left\| \mathbf{r}_N - \mathbf{r}_{target} \right\|_2 } 
         { \left\| \mathbf{r}_0 - \mathbf{r}_{target} \right\|_2} \right)^2
\end{equation}

\textbf{The overall cost function} will be a basic ingredient in all other proposed methods, we well refer to this function as \textbf{MPC}. This overall cost function is a sum of the stage cost and the terminal cost functions:

\begin{equation} 
    J_{MPC} = \sum_{{k_{c}}=0}^{N-1} J_{k_{c}} (\mathbf{u}_{k_{c}}, \mathbf{r}_{k_{c}}) + J_{N}\left(\mathbf{r}_{N}\right)
\end{equation}
Hence, the minimization problem that has to solved is:

\begin{equation} 
    \begin{aligned}
        & \min _{\mathbf{r}_{1: N}, \mathbf{u}_{0: N-1}} J_{MPC} = 
        \min _{\mathbf{r}_{1: N}, \mathbf{u}_{0: N-1}}
        \left(
        \sum_{k_{c}=0}^{N-1} J_{k_{c}} (\mathbf{u}_{k_{c}}, \mathbf{r}_{k_{c}}) + J_{N}\left(\mathbf{r}_{N}\right)
        \right), \\ 
        & \text{s.t. } \mathbf{r}_{0}=\mathbf{r}(0) \\
        & \mathbf{u}_{k_{c}} \in \mathcal{U}, \quad \mathbf{x}_{k_{c}} \in \mathcal{S}
    \end{aligned}
\end{equation}
% where:
% \begin{itemize}
%     \item[] \(\mathcal{U} \)- action space;
%     \item[]\( \mathcal{S} \)- state space;
% \end{itemize}

In summary, the described above formulas form the core of the problem. 

Next, we introduce additional elements for the formulated problem:
Euclidean Distance is a classical constraint that we add as an additional ingredient to\textit{ the stage cost function}:

\begin{equation} 
J_{k_{c}}^{\mathbf{ED}} (\mathbf{r}_{k_{c}}, \mathbf{p}^1_{k_{c}}, \mathbf{p}^2_{k_{c}}, ..., \mathbf{p}^{N_{ped}}_{k_{c}} ) = Q_{\mathbf{ED}} \sum_{i=0}^{N_{ped}} \frac{1}{
            \left\| \mathbf{r}_{k_{c}} - \mathbf{p}^i_{k_{c}} \right\|
}
\end{equation}

Hence, the minimization problem of the overall cost function with an Euclidean distance term will look like:
\begin{equation} 
    \begin{aligned}
        & \min _{\mathbf{r}_{1: N}, \mathbf{u}_{0: N-1}} J_{ED-MPC} = 
        \min _{\mathbf{r}_{1: N}, \mathbf{u}_{0: N-1}}
        \left(
        \sum_{k_{c}=0}^{N-1} \left( J_{k_{c}} (\mathbf{u}_{k_{c}}, \mathbf{r}_{k_{c}}) +
J_{k_{c}}^{\mathbf{ED}} (\mathbf{r}_{k_{c}}, \mathbf{p}^1_{k_{c}}, \mathbf{p}^2_{k_{c}}, ..., \mathbf{p}^{N_{ped}}_{k_{c}} ) \right)+ J_{N}\left(\mathbf{r}_{N}\right) 
        \right), \\ 
        & \text{s.t. } \mathbf{r}_{0}=\mathbf{r}(0) \\
        & \mathbf{u}_{k_{c}} \in \mathcal{U}, \quad \mathbf{x}_{k_{c}} \in \mathcal{S}
    \end{aligned}
\end{equation}
We will refer this cost function as \textbf{ED-MPC} as Euclidean distance (as an additional component to the base cost function )

Also, Euclidean distance could be added not only in the cost function, but as a inequality constraint function with some lower boundary :

\[
c^{\mathbf{ED}}_{k_{c} | i}\left(\mathbf{r}_{k_{c}}, \mathbf{p}_{k_{c}}^{i}\right)= \left\| \mathbf{r}_{k_{c}} - \mathbf{p}^i_{k_{c}} \right\| \geq r^{robot}+r^{ped}+d^{safe},
\]
The optimization problem of the basic MPC controller with added Euclidean distance constraint will have such formulation \ref{eq:MPC-EDC-cost}:

\begin{equation} 
    \begin{aligned}
        & \min _{\mathbf{r}_{1: N}, \mathbf{u}_{0: N-1}} J_{MPC-EDC} = 
        \min _{\mathbf{r}_{1: N}, \mathbf{u}_{0: N-1}}
        \left(
        \sum_{k_{c}=0}^{N-1} J_{k_{c}} (\mathbf{u}_{k_{c}}, \mathbf{r}_{k_{c}}) + J_{N}\left(\mathbf{r}_{N}\right)
        \right), \\ 
        & 
c^{\mathbf{ED}}_{k_{c} | i}\left(\mathbf{r}_{k_{c}}, \mathbf{p}_{k_{c}}^{i}\right)= \left\| \mathbf{r}_{k_{c}} - \mathbf{p}^i_{k_{c}} \right\| \geq r^{robot}+r^{ped}+d^{safe}, \\
        & \text{s.t. } \mathbf{r}_{0}=\mathbf{r}(0) \\
        & \mathbf{u}_{k_{c}} \in \mathcal{U}, \quad \mathbf{x}_{k_{c}} \in \mathcal{S}
    \end{aligned}
\end{equation}
We will refer this controller as a \textbf{MPC-EDC} read as basic MPC with an Euclidean distance constraint.

Combining Euclidean distance in the cost function and Euclidean distance in the constraint function we can achieve \textbf{ED-MPC-EDC }controller. Later, we will compare the results on the performance of them.

In addition we are introducing an adaptive constraint:

Here we describe our base controllers based on MPC: Euclidean cost, Euclidean constraint, Mahalanobis cost, Mahalanobis constraint. We put references, motivation and derivations.
\textbf{d}
We also put here how we embed the CovarianceNet and our approach with "ghosts" tracking. Probably also emphasize here that we do detection with realistic limited field of view, unlike many other papers.

We also can show in this section that our MPCs with global goals struggle with many scenes.

\subsection{Subgoal evaluation}

Here we describe our approach for subgoal evaluation: what is the input and what is the output of the network, what we predict. Then we show how it influence the performance of the controllers if we do kind of naive sampling of subgoal candidates.

\subsection{Formulas(Temporary)}
Euclidean constraint:
\[
c_{k}^{i}\left(\mathbf{x}_{k}, \mathbf{x}_{k}^{i}\right)=\left\|\mathbf{p}_{k}, \mathbf{p}_{k}^{i}\right\| \geq r+r_{i}+r_{s},
\]

State unattainability cost:
\[
J_{N}\left(\mathbf{p}_{N}, \pi(\mathbf{x}, \mathbf{X})\right)=\left\|\frac{\mathbf{p}_{N}-\mathbf{p}_{0}^{\text {ref }}}{\mathbf{p}_{0}-\mathbf{p}_{0}^{\text {ref }}}\right\|_{Q_{N}}
\]

Control penalty cost:
\[
J_{k}^{\mathbf{u}}\left(\mathbf{u}_{k}\right)=\left\|\mathbf{u}_{k}\right\|_{Q_{u}}, \quad k=\{0,1, \ldots, N-1\},
\]

Regular MPC formulation:
\[
\begin{aligned}
\min _{\mathbf{x}_{1: N}, \mathbf{u}_{0: N-1}} & J_{N}\left(\mathbf{x}_{N}, \mathbf{p}_{0}^{\text {ref }}\right)+\sum_{k=0}^{N-1} J_{k}^{u}\left(\mathbf{u}_{k}\right) \\
\text { s.t. } & \mathbf{x}_{0}=\mathbf{x}(0), \quad(1 \mathrm{~d}),(2) \\
& c_{k}^{i}\left(\mathbf{x}_{k}, \mathbf{x}_{k}^{i}\right)>r+r_{i}+r_{s} \\
& \mathbf{u}_{k} \in \mathcal{U}, \quad \mathbf{x}_{k} \in \mathcal{S} \\
& \forall i \in\{1, \ldots, n\} ; \forall k \in\{0, \ldots, N-1\} .
\end{aligned}
\]

The probability of collision is approximately given by:
$$
\begin{aligned}
P(C) \approx & V_{\mathcal{S}} \times \frac{1}{\sqrt{\operatorname{det}\left(2 \pi \Sigma_{C}\right)}} \\
& \times \exp \left[-\frac{1}{2}\left(\hat{x}_{R}-\hat{x}_{A}\right)^{T} \Sigma_{C}^{-1}\left(\hat{x}_{R}-\hat{x}_{A}\right)\right]
\end{aligned}
$$

Equivalent constraint:

$$
\begin{aligned}
\left(\hat{x}_{R}-\hat{x}_{A}\right)^{T} \Sigma_{C}^{-1}\left(\hat{x}_{R}-\hat{x}_{A}\right) & \geq-2 \ln \left(\sqrt{\operatorname{det}\left(2 \pi \Sigma_{C}\right)} \frac{\delta}{V_{\mathcal{S}}}\right) \\
& \triangleq \kappa
\end{aligned}
$$

Lemma 4:
\begin{equation}
P\left(\|\mathbf{x}\|^2 \leq \alpha\right) \leq F_{c h i}^{-1}\left(\lambda_{\max }\left(\alpha-2 \mathbf{x}^T \boldsymbol{\mu}+\boldsymbol{\mu}^T \boldsymbol{\mu}\right)\right)
\end{equation}

% Compact Robot Dynamics Equations
\begin{equation}
     \mathbf{x}_{k+1} = \mathbf{x}_k + 
     \begin{bmatrix}
       cos(\theta^{rob}_k) & 0        \\[0.3em]
       sin(\theta^{rob}_k) & 0        \\[0.3em]
       0                   & 1
     \end{bmatrix}
     \mathbf{u}_k \Delta t
\end{equation}

% % MPC-AEDC
% \begin{equation} \label{eq:MPC-AEDC}
%     \resizebox{\resizecoef\columnwidth}{!}{
%         \begin{aligned}
%             & \underset{\mathbf{r}_{1: H}, \bar{\mathbf{u}}_{0: H-1}}{\text{min}}
%             & &\sum_{k=0}^{H-1} ( J_{k} (\bar{\mathbf{u}}_{k}, \mathbf{r}_{k})
%                 + J_{H}\left(\mathbf{r}_{H}\right) \\
%             & \text{subject to}
%             & & \mathbf{r}_{0}=\mathbf{r}(0)  \\
%             &&& d^{\mathbf{ED}}_{k, i}\left(\mathbf{r}_{k}, \mathbf{p}_{k, i}\right) \geq r^{rob}+r^{ped}+d^{safe}+\delta \\
%             &&& \bar{\mathbf{u}}_{k} \in \bar{\mathbb{U}} \\
%             &&& \mathbf{r}_{k} \in \mathbb{W}
%         \end{aligned}
%     }
% \end{equation}

% % MD-MPC-AMDC
% \begin{equation} \label{eq:MD-MPC-AMDC}
%     \resizebox{\resizecoef\columnwidth}{!}{
%         \begin{aligned}
%             & \underset{\mathbf{r}_{1: H}, \bar{\mathbf{u}}_{0: H-1}}{\text{min}}
%             & &\sum_{k=0}^{H-1}  J_{k} (\bar{\mathbf{u}}_{k}, \mathbf{r}_{k})
%                 + J_{H}\left(\mathbf{r}_{H}\right) \\
%             & \text{subject to}
%             & & \mathbf{r}_{0}=\mathbf{r}(0)  \\
%             &&&  d^{\mathbf{MD}}_{k, i}\left(\mathbf{r}_{k}, \mathbf{p}_{k, i}\right) \geq 2 \ln \left(\sqrt{\operatorname{det}\left(2 \pi \Sigma_{k , i}\right)} \frac{P^{col}}{V^{rob}}\right) + \delta \\
%             &&& \bar{\mathbf{u}}_{k} \in \bar{\mathbb{U}} \\
%             &&& \mathbf{r}_{k} \in \mathbb{W}
%         \end{aligned}
%     }
% \end{equation}

==> unused_materials.tex <==
% Common Parameter Table
\begin{table}[]
\centering
\label{tab:common-parameter-table}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll}
\(N \in \{3, 4, 5, 6, 7, 8\} \)        & \(\Delta t^{sim} = 0.01\)  & $d^{safe} = 0.3 $          \\
\(H = 25\)                             & $H^{ghost} = 20 $        & $\varepsilon = 0.3$         \\
\(\Delta t = 0.1\)                     & $r^{rob} = 0.35 $  & $\ell^{vis} = 5$          \\
\(T^{sim} = 2000\)                     & $r^{ped} = 0.3  $ &  $\varphi^{vis} = 2\pi$           
\end{tabular}         
}
\end{table}
